Code Search Debiasing:Improve Search Results beyond Overall Ranking Performance

Code search engine is an essential tool in software development. Many code search methods have sprung up, focusing on the overall ranking performance of code search. In this paper, we study code search from another perspective by analyzing the bias of code search models. Biased code search engines provide poor user experience, even though they show promising overall performance. Due to different development conventions (e.g., prefer long queries or abbreviations), some programmers will find the engine useful, while others may find it hard to get desirable search results. To mitigate biases, we develop a general debiasing framework that employs reranking to calibrate search results. It can be easily plugged into existing engines and handle new code search biases discovered in the future. Experiments show that our framework can effectively reduce biases. Meanwhile, the overall ranking performance of code search gets improved after debiasing.

==> texs/method.tex <==
%!TEX root = ../main.tex

\section{Method}


We have analyzed some bias in multifarious deep learning based code search models, 
which will be described in this section. 
We have chosen four typical code search models: CODEnn, CQIL, 
CodeBERT, and CoCLR for bias analysis. They are all briefly described 
in the “related work” section. 

We use MRR as the evaluation index, 
which can visualize the search performance of the model. 
It can be described as follow:
\[
    MRR = \frac{1}{Q} \sum_{i=1}^Q \frac{1}{rank_i}
\]
Among them, Q indicates the number of data, 
and $rank_i$ suggests the order of the correct data in the model output list. 
For example, when the correct result is ranked 2nd, the value of MRR is 1/2, 
which is 0.5.

\subsection{Code Search Bias Analysis}
\subsubsection{Code Length Bias}
We assume that longer code can provide more semantic information. 
Models will get higher MRR when facing long code. For the test data, 
we sorted them by code length and plotted the “CodeLength-MRR” curve chart.
The left vertical axis indicates the number, 
which shows how much data are in each interval. 
The right vertical axis indicates the average MRR of the model 
when tested with data from different intervals. 
The horizontal axis indicates the length of the code, 
in intervals of 4 and in ascending order.
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{images/CQILCodeLen.jpg}
    \caption{CQILCodeLen\label{CQILCodeLen}}
\end{figure}

Figure~\ref{CQILCodeLen} shows the code length bias in the four code search baseline models.

\subsubsection{Query Length Bias}
Like code length bias, long natural queries can contain more information. 
The “QueryLength-MRR” curve chart is shown as follows.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{images/CQILQueryLen.jpg}
    \caption{CQILQueryLen}
\end{figure}

\subsubsection{AST Length Bias}
Converting code into an AST(abstract syntax tree) is 
an important part of code compilation. The shape of the AST 
for a given piece of code is determined by its structure. 
Usually, longer code has a deeper one, while some complex short code, 
such as list parsing in python syntax, also gets a complex tree. 
We analyzed the impact of code AST depth and the number of AST nodes 
on model performance.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{images/CQILAstLevel.jpg}
    \caption{CQILAstLevel}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{images/CQILAstNode.jpg}
    \caption{CQILAstNode}
\end{figure}

\subsubsection{Typical Query Word Bias}
If natural queries contain some meaningful and directed words, 
models may easily find semantically related codes. For each query, 
we calculated the max TF-IDF value and average TF-IDF value of each term. 
Then, we sort test data by these two factors and observe the change in MRR 
as the two rises. 

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{images/CQILTfidfA.jpg}
    \caption{CQILTfidfAverage}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{images/CQILTfidfM.jpg}
    \caption{CQILTfidfMax}
\end{figure}

\subsection{Debias Method based on Reranking}

In this section, we propose a debias method based on reranking. 
Reranking is a method for optimizing a list of existing results. 
The model outputs a series of results, usually ordered by score, 
which may have some bias or ignore the overall association between items. 
Therefore, the results can be re-ranked according to some rules 
to improve performance or remove bias.Our Reranking method is motivated by (\citealp{AbdollahpouriBM19}). 

The reordering method we used in this section is defined as Eq~\ref{eq:Reranking}. 
The core idea of this formula is to add a regularization score for 
candidate codes whose length is less than the length threshold.

\begin{footnotesize}
\begin{equation}
    R_{score} =
    \begin{cases}
    O_{score} + \lambda(\frac{1}{P(C^\prime|C)}+\frac{1}{P(C^\prime|R^\prime)}) & \text{if } x < 0\\
    O_{score} & \text{if } C^\prime > Len\\
    \end{cases} 
    \label{eq:Reranking}
\end{equation}
\end{footnotesize}

Among them, $Len$, $\lambda$ are hyperparameters. 
$O_{score}$ is the original score in the sorted list generated by the model. 
$C^\prime$ represents the code whose length is less than or equal to $Len$, 
$C$ represents the overall code, 
and $R^\prime$ represents the test data of which the correct answer 
in the origin results is higher than a threshold rank. 
We use the average correct answer rank as the threshold.
before the rearrangement is greater than the average ranking of all correct results. 
data. 
$\lambda$ usually depends on the code search model. For different models, the order of magnitude of $\lambda$ will be different. 

Our experiments found that rerank all the test data may damage 
the model performance because only the short code data needs to be rerank. 
Therefore, we proposed a length prediction network 
whose role is to determine the results of a given query 
whether it needs rerank or not. The details are as follows. 
For a query statement q, the length of its corresponding 
correct answer is predicted using the length prediction network, 
and if this length is less than the length threshold $L$, 
the result list will be rerank, and if the predicted length is greater than $L$, 
it will not be rerank.

We treat the length predict problem as a binary classification. 
The network's output determines whether the search result of a query 
needs to be rerank. The structure is illustrated in Figure~\ref{codePreNet}. 
A query will be first encoded by a CodeBERT and then classified by an MLP. 
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.5]{images/codePreNetwork.png}
    \caption{codePreNetwork\label{codePreNet}}
\end{figure}


\subsection{Data Preprocess}
At present, the mainstream code search datasets mainly include the following:

(1) CodeSearchNet dataset [21]. This dataset is provided on the 
Code Search Challenge published by Github. 
The dataset includes nearly 6 million functions, 
covering six programming languages: Go, Java, JavaScript, PHP, Python, and Ruby.

(2) CODEnn dataset [3]. This dataset is the "Code-Annotation" dataset 
collected by the researchers on the Github repository. 
It is in Java language and contains 18,233,872 pieces of data. 
The researchers used the collected Java functions as code, 
and the documentation comments of the function as the natural language description 
of the corresponding code.

(3) CoSQA dataset [11]. The data set is a Python language data set, 
covering 20,604 pieces of data. The researchers manually corresponded 
the codes to the real query sentences one-to-one.

This paper selects the CoSQA dataset for experiments and analysis. 
The reasons are as follows:
(1) The quality of the dataset is high, 
and each piece of data is manually labeled. Unlike other datasets 
that use annotations as descriptions, this dataset uses real query statements 
to correspond to codes.
(2) The number of data sets is small, which is convenient for 
large-scale experiments in bias analysis.
The fields of the CoSQA dataset are shown in Table 3.1.
\begin{table*}
    \centering
    \begin{tabular}{lll}
    \hline
    \textbf{token name} & \textbf{data type} & \textbf{data mean}\\
    \hline
    idx & string & aa \\
    doc & string & aa \\
    code & string & aa \\
    code\_tokens & string & aa \\
    docstring\_tokens & string & aa \\
    label &  int & aa\\
    \hline
    \end{tabular}
    \caption{\label{citation-guide}
    Citation commands supported by the style file.
    The style is based on the natbib package and supports all natbib citation commands.
    It also supports commands defined in previous ACL style files for compatibility.
    }
\end{table*}

For the dataset, it is preprocessed as follows:

First, extract the data whose field label is 1 and the data whose label is 0. 
The former indicates that the query statement is related to code semantics, 
while the latter indicates that the semantics are irrelevant. 
Only semantically matching data needs to be considered in the test set. 
Next, divide it by 7:3. Among them, 70\% and the label 0 data are combined and scrambled and used as training data, and the remaining 30% are used as test data.

Second, the data is processed into the input form corresponding to each baseline model.

The input form of CodeBERT and CoCLR is similar to that of BERT, as shown in (3.1),
\[
    \left[cls\right],c_1,c_2,c_3,\left[sep\right],,n_1,n_2,n_3...\left[eos\right]
\]
% ([cls],c_1,c_2,c_3...[sep],n_1,n_2,n_3...[eos]) (3.1)

Among them, c\_1, n\_1 represent code characters and query statement characters. 
% [cls], [sep], [eos], are the separators for marking the position. 
Here, with the help of the tokenizer (Tokenizer) provided by the Transformer module, 
the code segment and the query statement are converted into the above format.

The original dataset of CODEnn and CQIL methods is Java language, 
which is quite different from the CoSQA dataset selected in this paper. 
CODEnn data input format is function name, function Api call list, 
function body field Tokens and natural language description. 
CQIL method data input format is function name, function body field and 
natural language description.

To extract the function Api call sequence, you need to use the Python AST module.

To extract the function body field, select the Python tokenize module to parse 
and segment the code.

\subsection{Evaluation Index MRR}
This paper uses MRR to evaluate code search performance. 
The core idea of MRR is to evaluate the performance of the system 
by the ranking of the correct result among all the results. 
Its definition is given as follow:
\[
    MRR = \frac{1}{Q} \sum_{i=1}^Q \frac{1}{rank_i}
    \]

Among them, Q indicates the number of data, 
and rank\_i indicates the order of the correct data in the current model input. 
For example, when the correct result is ranked 2nd, the value of MRR is 1/2, 
which is 0.5.

Using MRR as the evaluation index can intuitively see the performance of the 
code search model. 
The larger the MRR, the more accurate the search results.

\subsection{Baseline Model Performance Testing}
The performance of the four baseline models on the test dataset is shown in Figure.

It can be seen from the results that CodeBERT and CoCLR perform better, 
while CQIL and CODEnn perform poorly. 
Although the performance of CQIL, CODEnn methods is less than ideal, 
it is also within the acceptable range. This article believes 
that the reasons may be as follows:

(1) The two methods of CodeBERT and CoCLR are pre-training models. 
The network structure is based on the Transformer encoder and 
uses a multi-head attention mechanism. The performance of the attention mechanism 
in various fields shows that it is better than the convolutional neural network 
and the recurrent neural network. have better effect;

(2) The original data set of CQIL and CODEnn is a Java data set, 
and the data volume is much larger than that of the CoSQA data set. 
Generally, programs written in Java language are longer 
than those written in Python language, and more information can be 
obtained by obtaining function call APIs and function body field tokens.

(3) The CQIL and CODEnn methods do not provide the code for extracting 
the function call Api and the function body field tokens. 
Only the general method is introduced in the relevant papers. 
In the processing method of the data set, 
the method in this paper may be inappropriate. 

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.4]{images/baselineTest.png}
    \caption{Average MRR of the four baseline models}
\end{figure}

\subsection{Code Length Bias and Debias}
Code search models learn the semantic relevance between natural language queries 
and program code. Generally, for a code search model, 
its loss function is expressed as:
\[
    L=(1-Sim(E_+, C_+)+Sim(E_-, C_-))
\]

Among them, Sim represents similarity. 
E\_+ and C\_+ represent semantically matching codes, 
usually a piece of data in the training set. And E\_-, C\_-, 
it means the code that does not match semantically, 
usually use random sampling to get.
Data with longer code length can provide more semantic information, 
and it is easier for the model to match it with the corresponding query statement, 
which provides support for our analysis of length deviation.

This section conducts a length bias analysis on the four baseline models. 
This section expands the analysis through the following methods:
First, count the length of the longest code in the test data set, 
and divide it into several intervals according to the length of 4. 
Next, count the average MRR in each interval and the number of samples in that interval. 
Finally, draw the "MRR-length" graph in the order of increasing length, 
and observe whether there is a correlation between the value of MRR and the code length.
The "MRR-Length" plots are plotted for the four models according to the method 
described above, as shown in Figures 3.2-3.5. The horizontal axis is the code length, 
with 4 as the interval, the left vertical axis corresponds to the bar chart, 
indicating how many pieces of data there are in each length interval, 
and the right vertical axis represents the MRR value.

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.3]{images/CQILBeforeDebias.png}
%     \caption{CQILBeforeDebias}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.3]{images/CODEnnBeforeDeibas.png}
%     \caption{CODEnnBeforeDeibas}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.3]{images/CodeBERTBeforeDebias.png}
%     \caption{CodeBERTBeforeDebias}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.3]{images/CoCLRBeforeDebias.png}
%     \caption{CoCLRBeforeDebias}
% \end{figure}


It can be seen from the figure that the CQIL method 
has a relatively obvious length deviation. 
When the code length is in the interval of 45 to 65, 
the model performance is better, 
which is higher than that of the data whose length is less than 45; 
the length deviation of the CODEnn method is not obvious. 
When the code length is close to 60, the model performance is slightly improved. 
The possible reason is that the model input is the function call API 
and the function body field Tokens, 
which weakens the impact of the length to some extent; 
the CodeBERT model also has obvious problems. In the CoCLR method, 
when the code length is shorter, the model performance decreases 
with the increase of the code length, and when the code length is close to 55, 
the model performance decreases. There is a more obvious increase. 
In general, in CoCLR, the performance of long code data model is better than 
that of short code data, so there is also the phenomenon of length deviation.

To sum up, the code search model generally has the phenomenon of length deviation, 
that is, as the length of the candidate code increases, 
the performance of the model will also increase accordingly.

\subsection{Debias based on Reranking}
In this section, we propose a debiasing method based on reranking. 
Reranking is a method for optimizing the existing recommendation ranking 
in the recommender system. For a user, the recommender system recommends a series of 
items sorted by score, 
and the unoptimized ranking may be biased or 
ignore the overall correlation between items. Therefore, 
the existing recommendation list can be reordered according to certain 
rules to improve recommendation performance or remove bias.

The reordering method used in this section is defined as shown in Equation. 
The core idea of this formula is to add a regularization score to 
the candidate code whose length is less than the length threshold Len.


Among them, Len, $\lambda$ are hyperparameters. 
$O_{score}$ is the score of each list item in the sorted list generated by the model 
before reordering, $C^\prime$ represents the code whose length is less than or equal to Len, 
C represents the overall code, and $R^\prime$ represents the correct result 
before the rearrangement is greater than the average ranking of all correct results. 
data. $\lambda$ usually depends on the evaluation index adopted by the original model. 
Different evaluation indicators will affect the magnitude of . For example, 
when the probability of semantic similarity is used as the evaluation system 
and the binary classification is used as the evaluation system, the data magnitude 
of will be quite different.

